Large-scale Gender/Age Prediction of Tumblr Users

Tumblr, as a leading content provider and social media, attracts 371 million monthly visits, 280 million blogs and 53.3 million daily posts. The popularity of Tumblr provides great opportunities for advertisers to promote their products through sponsored posts. However, it is a challenging task to target specific demographic groups for ads, since Tumblr does not require user information like gender and ages during their registration. Hence, to promote ad targeting, it is essential to predict user's demography using rich content such as posts, images and social connections. In this paper, we propose graph based and deep learning models for age and gender predictions, which take into account user activities and content features. For graph based models, we come up with two approaches, network embedding and label propagation, to generate connection features as well as directly infer user's demography. For deep learning models, we leverage convolutional neural network (CNN) and multilayer perceptron (MLP) to prediction users' age and gender. Experimental results on real Tumblr daily dataset, with hundreds of millions of active users and billions of following relations, demonstrate that our approaches significantly outperform the baseline model, by improving the accuracy relatively by 81% for age, and the AUC and accuracy by 5\% for gender.

==> 051experiments_production.tex <==
\section{Deployed System}
\label{sec:production}



\subsection{Input Datasets}
All the data is presented as hive tables. The Tumblr follower information is from \textcolor{red}{\texttt{urs\_prd.tumblr\_user\_follows}}. This data is then preprocessed to remove very inactive tumblr users i.e., users who follow less than 25 blogs. The cumulative feature is from \textcolor{red}{\texttt{urs\_prd.tumblr\_features\_cumulative}}. As we mentioned above, we leverage Yahoo's device ID to create reliable labels.

%The tumblr labelled data was created using an overlaap between tumblr users, and Yahoo mail users , since the quality of tumblr declared demographic information is very poor.  

\subsection{Feature Engineering}
\noindent \textbf{Label propagation features for gender.} 
%We create a bidirectional graph of the tumblr users, where a connection between two nodes i.e. tumblr users represents a follow or followed relationship. This graph has roughly about 150 Million nodes and 12 Billion edges. In this graph we then use our labelled data to add the labels for some of the nodes. 
As mentioned above, we implemented \lp using the Pregel framework on Spark in production, 
with the following specifications:  \emph{Number of Iterations: 3; $\alpha$, the fraction of the current label: 0.3; Number of splits: 3}. We split the data into 3 parts to generate graph based features. %over the labels propagated from the three splits. This kind of avoids over fitting.

\smallskip
\noindent \textbf{Embedding features for age.} 
The tumblr user followers are arranged in the form of a document, where each document starts with a tumblr user , and followed by all the users whom he follows or who follow him ($\sim$150 Million lines in total).  We then run PS-Word2Vec built by the Big ML team, with the following specifications: \emph{Model type: Continuous Bag of Words; Bi-directional Window size: 6, i.e. 6 words on each side of a user are chosen as the context for training; Minibatch size: 100; Epoch Count: 1}. The training process takes around 3 hours. 

%The tumblr user followers are then arranged in the form of a document, where each line starts with a tumblr user , followed by all the users whom he follows or who follow him (~ 150 Million lines in total).  We then run a word 2 vector model built by the Big ML team, here at Yahoo on it with the following specifications ( Model type : Continuous Bag of Words , Bi-directional Window size : 6 i.e. 6 words on each side of a user are chosen as the context for training , Minibatch size : 100, Epoch Count : 1). This word 2 vec training takes around 3 hours. 

\subsection{Modeling}

\noindent \textbf{Training and testing split.}
We use features created for each tumblr blog Id above, and join them with labels, which generates about 3.5 million labeled data. We then split this data into training and testing parts ($75\%$, $25\%$), based on the hash of tumblr Ids. This way the training and testing set are deterministic, i.e., these sets are always separated. In addition, they can both grow in the same ratio with the addition of new tumblr users.

\smallskip

\noindent \textbf{Deep learning models.}
We implement our approaches using \textcolor{red}{Tensorflow on Spark built by the Big ML team}. Currently we have pushed \mlp into production. In production, we train and and update our model everyday using Oozie. This helps us avoid the model getting outdated over time, and requiring periodic manual retraining. The deep learning model has the following specifications: \emph{Architecture: 3 layers neural network with each layer having 256 Neurons; Loss Function: Cross Entropy Loss; Epoch Count: 4; Minibatch size: 3000}. This model produced a testing accuracy of $36\%$ on average. The model takes roughly 30 minutes to train, and 10 minutes for evaluation. 

%\noindent \textbf{Train and Test Datasets.}
%We use the features created for each tumblog Id above , and join it with the tumblr labelled data. This creates the input training data (~ 3.5 Million). We then split this data into train and test set (75\%, 25\%), based on the hash of the tumblr user id ( This way the train and test set is deterministic i.e These sets are always seperate and they both also grow in the same ratio with the addition of new tumblr users as well.)

%\subsection{Deep Learning Classification Model}
%We then use tensorflow on spark built by the Big ML team , to run our tensorflow model for training. We train the model and evaluate the data on the test set everyday using Oozie. This helps us avoid the model getting stale over time, and requiring periodic manual retraining. The deep learning model has the following specifications ( Architecture : 3 layers neural network, with each layer having 256 Neurons, Loss Function :  Softmax Cross Entropy Loss , Epoch Count: 4 , Minibatch size : 3000 , Training Data Size : 2.6 Million). This model produced an accuracy of 36\% on average on the test set ( ~ 800k users) . The model takes roughly 30 minutes to train , and 10 minutes for evaluation. 

%\subsection{Combine Age and Gender Predictions}

\subsection{Deployment}
We combine the age and gender predictions to obtain the final result and store in the Hive table \textcolor{red}{(\texttt{urs\_prd.urs\_tumblr\_demo})}, as the final step.



==> makefile <==
RCSFLAGS= -l
MAIN= paper
TEXPARTS= 010intro.tex \
	020prelim.tex \
	030formulation.tex \
	040method.tex \
	050experiments.tex \
	060related.tex \
    070conclusion.tex 
BIBPARTS= BIB/*.bib
LPR = pspr # or change to 'qpr -q ps3'
POSTSCRIPT= dvips -f
FIGPARTS= FIG/*.eps FIG/*.pdf FIG/*.fig FIG/*.jpg FIG/*.png
STYPARTS= vldb.cls
MISC= makefile README
LATEX= pdflatex

# $(MAIN).pdf: $(MAIN).dvi
# 	$(POSTSCRIPT) $(MAIN).dvi > $(MAIN).ps

$(MAIN).pdf: $(MAIN).tex $(TEXPARTS) $(BIBPARTS)
	$(LATEX) $(MAIN).tex
	bibtex $(MAIN)
	$(LATEX) $(MAIN).tex
	$(LATEX) $(MAIN).tex

# print: $(MAIN).ps
# 	$(LPR) $(MAIN).ps


clean:
	rm -f *.synctex.gz  *.dvi *.pdf $(MAIN).ps *.bbl *.aux *.log *.blg *.toc all.tar* uu \
	*~ *.bak 

spotless: clean
	rm -f $(MAIN).ps $(MAIN).pdf
	rm -rf TST


all.tar:
	tar cvfh all.tar $(MAIN).tex $(TEXPARTS) $(BIBPARTS) \
	$(FIGPARTS) $(STYPARTS) $(MISC)

dt: spotless
	dotest

uu: all.tar
	gzip all.tar
	uuencode all.tar.gz all.tar.gz > uu

bundle.all: $(TEXPARTS) 
	bundle  README $(TEXPARTS) $(BIBPARTS) makefile > bundle.all

